First Light And Reionisation Epoch Simulations (FLARES) XII: The consequences of star-dust geometry on galaxies in the EoR

Using the First Light And Reionisation Epoch Simulations (${\rm F{\small LARES}}$), a suite of hydrodynamical simulations we explore the consequences of a realistic model for star--dust geometry on the observed properties of galaxies. We find that the UV attenuation declines rapidly from the central regions of galaxies, and bright galaxies have spatially extended star formation that suffers less obscuration than their fainter counterparts, demonstrating a non-linear relationship between the UV luminosity and the UV attenuation, giving a double power-law shape to the UVLF. Spatially distinct stellar populations within galaxies experience a wide range of dust attenuation due to variations in the dust optical depth along their line-of-sight; which can range from completely dust obscured to being fully unobscured. The overall attenuation curve of a galaxy is then a complex combination of various lines-of-sight within the galaxy. We explore the manifestation of this effect to study the reliability of line ratios to infer galaxy properties, in particular the Balmer decrement and the BPT diagram. We find the Balmer decrement predicted Balmer line attenuation to be higher (factor of $1$ to $\gtrsim10$) than expected from commonly used attenuation curves. The observed BPT line ratios deviate from their intrinsic values (median difference of 0.08 (0.02) and standard deviation of 0.2 (0.05) for log$_{10}$([N${\rm {\small II}}$]$\lambda 6585/$H$_{\alpha}$) (log$_{10}$([O${\rm {\small III}}$]$\lambda 5008/$H$_{\beta}$)). Finally, we explore the variation in observed properties (UV attenuation, UV slope and Balmer decrement) with viewing angle, finding average differences of $\sim0.3$ magnitudes in the UV attenuation.

==> limitations.tex <==
\section{Limitations of this work}\label{sec:lim}
\begin{itemize}
    \item We donot know the intrinsic attenuation curve and assumes one
    \item Related to that there will be evolution in grain properties
\end{itemize}

==> results.tex <==
\section{Results}\label{sec:results}
In this section we will show some of the results from our analysis, starting with the spatial variation and then due to different line-of-sights.

\subsection{Radial variation}\label{sec: rad var}
\begin{figure*}
	\includegraphics[scale=0.41]{figures/att_radial_var_mstar_aperture.png}
	\includegraphics[scale=0.41]{figures/att_radial_var_mstar_annuli.png}
	\caption{Left: The variation of the far-UV attenuation within apertures that are multiple of the galaxy UV half-light radius for different stellar mass bins. Right: Same plot as on the left, but the attenuation is calculated within different annuli. The shaded region shows the 16th and 84th percentile. Only bins with more than 5 galaxies are shown.\label{fig: att_rad_mstar}}
\end{figure*}
%\begin{figure*}
%	\includegraphics[scale=0.41]{figures/att_radial_var_fuv_aperture.png}
%	\includegraphics[scale=0.41]{figures/att_radial_var_fuv_annuli.png}
%	\caption{Left: The variation of the far-UV attenuation within apertures that are multiple of the galaxy UV half-light radius for different UV magitude bins. Right: Same plot as on the left, but the attenuation is calculated within different annuli. Only bins with more than 5 galaxies are shown.\label{fig: att_rad_fuv}}
%\end{figure*}

Using the half-light radii calculated in \S\ref{subsec: hlr} we describe how the average UV attenuation within galaxies vary with distance from the centre. In Figure~\ref{fig: att_rad_mstar}, we plot the radial variation of the median attenaution with the half-light radii multiples for $z\in[5,8]$. The left subplot shows this variation within apertures while the right subplot is for different annuli. In the same plot we have shown by dashed lines the median attenuation within that galaxy bin. As expected the attenuation within apertures approach the median value as the size increases. However the median varies over by a 1.5 magnitude radially from the global value. An interesting feature here is the dramatic offset between the lowest mass bins and the rest. This feature has also been seen in observations pointing towards the rapid build of dust in the highest mass galaxies £cite£. If one examines the right subplot, it is obvious that the bulk of the stellar light within the central region suffers the most attenuation, following almost an exponential decay towards the half-light radii, to approach the median. This behaviour is confirmed in the right plot, where we can see this exponential decay of the value of attenuation, with the stellar light suffering very little loss to dust beyond the half-light radii. What is clear is that the spread in the individual values are very high, once again not in favour of single attenuation values, as expected at these high redshifts where the galaxies are predicted to be clumpy (citations). This would beed to be in consideration when extracting the relative contribution of obscured and unobscured star formation at high-redshifts, since applying a single global value underestimates the contribution of the highly obscured centre. 

%In Figure~\ref{fig: att_rad_fuv}, is the same figure as before, but the galaxies are split into bins based on their UV magnitude. Here one can see that the attenautions are closely related than what was the case with the stellar mass. As seen in Figure~9 in \cite{Vijayan2021}, the most attenuated galaxies are not the most brightest. But overall we see the same behaviour as before as expected. 


%A simple excercise to see the effect of such a spread in attenuation would be to see how much effect this has on the inferred fraction of obscured and unobscured star formation rate within the galaxy. In Figure~££, we look the relationship of the obscured star formation under assumptions of single values compared to a progressively declining values in different annuli.

%
%\begin{figure*}
%	\centering
%	\includegraphics[scale=0.6]{figures/fesc_distr_mass_fuv_z5.0.png}
%	\caption{text \label{fig: fesc_distr_z5}}
%\end{figure*}
%\begin{figure}
%	
%In the histogram plotted in Figure~\ref{fig: fesc_distr_z5}, we can see the dramatic increase in the dust content due to rapid star formation and dust enrichement within the centres of high mass galaxies. We can see that star particles within galaxies are either mostly present in the central dense clump which are becoming highly obscured (f$_{\mathrm{esc}}\sim 1$) with the galaxy stellar mass or outside the central region suffering very little attenaution f$_{\mathrm{esc}}\sim 0$. There is a negligible population of stars with intermediate values of the escape fraction.

\begin{figure*}
	\centering
	\includegraphics[scale=0.7]{figures/fesc_precentile_diff_mass_z.png}
	\caption{text \label{fig: fesc_distr_z5_8}}
\end{figure*}


Figure~\ref{fig: fesc_distr_z5_8} shows the spread in the attenuation faced by the different stellar particles, described by the difference between the 84th and 16th percentile, within the galaxy as a function of stellar mass, coloured by the global value of the attenuation. This plot makes it clear that there is a huge spread within a single galaxy even when the global value is very low. Another feature you see is the movement of galaxies which show medium spread to very high spread in the values. Also seen is young galaxies due to rapid enrichment moving from the very low spread region to higher. In the massive \flares\, galaxies, there is either a large spread in the value or not irrespective of their stellar mass. We also found that this spread cannot be explained as a function of the galaxy stellar age or the star formation rate, and thus is a property of the distribution of dust within the galaxy as well as presence of young stars which are embedded in their birth clouds.



\subsection{Line-of-sight variation}\label{sec:los var}
Plot HEALPIX attenuation maps for a selection of individual galaxies. Add the axis of rotation as a line. 

\begin{figure}
	\includegraphics[scale=0.2]{figures/test_5_mollview}
	\includegraphics[scale=0.2]{figures/test_793_mollview}
	\caption{Healpix maps for different sightlines for some selected galaxies in our sample. The sightlines have been coloured by the galaxy UV attenuation. The blue and yellow lines denote the gas and stellar plane respectively of the galaxy disc based on the angular momentum of the corresponding particles. \label{fig: healpy_plots}}
\end{figure}
In $\S$\ref{subsec: reproject} we explained how by using \textsc{healpy} we calculate different line-of-sight re-projections. In Figure~\ref{fig: healpy_plots} we show the attenuation maps for the different line-of-sights for a selection of our galaxies. The sightlines have been coloured by the galaxy UV attenuation. The blue and yellow lines denote the gas and stellar plane respectively of the galaxy disc calculated based on the angular momentum of the corresponding particles. 

\subsubsection{Population Trends}

Measure P84-P16 of UV attenuation for every galaxy and plot as a function of stellar mass.

Not sure I like UV attenuation. We could use optical depth (almost as bad) or escape fraction instead.

Are there trends with stellar mass or average dust attenuation? 


In Figure~\ref{fig: beta_mstar_los_spread}, we plot the spread of the UV continuum slope ($\beta$) with stellar mass with the hexbins coloured by the median of the median $\beta$ value of the galaxies within that bin. Similarly we plot the spread in the FUV attenuation in Figure~\ref{fig: afuv_mstar_los_spread}. As can be seen there is a minimal trend with the $\beta$ slope values with stellar mass, where the spread increase to a maximum for increasing stellar mass, and then starts decreasing again. For the case of the UV attenuation, this trend is stronger, with variations of the order of $\sim0.3$ magnitudes. 

\begin{figure}
	\includegraphics[scale=0.4]{figures/beta_mstar_los_percentile_spread.png}
	\caption{Shows the spread (84-16 percentile) of $\beta$ values for different line-of-sights as a function of their stellar masses, coloured by the median $\beta$ within hexbins for $z\in[5,8]$. \label{fig: beta_mstar_los_spread}}
\end{figure}
\begin{figure}
	\includegraphics[scale=0.4]{figures/AFUV_mstar_los_percentile_spread.png}
	\caption{Same plot as Figure~\ref{fig: beta_mstar_los_spread}, now shows the spread in UV attenuation for different lines-of-sight. \label{fig: afuv_mstar_los_spread}}
\end{figure}

\subsubsection{Correspondence with axis of rotation}

We next correlate the attenuation with the axis of rotation. Is the attenuation stronger perpendicular to the axis of rotation? You'd expect so for a pure disk galaxy.

Before we complete this paper we probably want a disk galaxy paper!

In Figure~\ref{fig: afuv_kappa_los_spread} we plot the relationship between the spread in attenuation with the galaxy being discy. We parameterise the discyness of a galaxy by the use of $\kappa_{\mathrm{co}}$. This value in a nutshell quantifies the energy invested in ordered corotation (see \cite{Sales2012,Correa2017} for more details), where galaxies with $\kappa_{\mathrm{co}}\ge0.4$ can be termed as discs. As exepected the spread in attenuation across different line-of-sights is maximum when the galaxy is more discy (higher $\kappa_{\mathrm{co}}$ value). This can also be seen in Figure~\ref{fig: healpy_plots} where the maximum of the attenuation traces the line-of-sight corresponding to the plane of the disc in these galaxies. 

\begin{figure}
	\includegraphics[scale=0.4]{figures/AFUV_kappa_percentile_spread.png}
	\caption{Same plot as Figure~\ref{fig: afuv_mstar_los_spread}, now shows the spread in UV attenuation for different lines-of-sight as a function of $\kappa_{\mathrm{co}}$, a parameter which quantifies how discy a galaxy is. \label{fig: afuv_kappa_los_spread}}
\end{figure}


\subsection{Attenuation Curve}
Dust attenuation curves describe how the intrinsic emission (from stellar and nebular continuum) from a galaxy is changed based on the intervening dust at different wavelengths. Understanding attenuation curves are required for robust determination of galaxy physical properties and thus crucial to galaxy formation and evolution studies. 


The attenuation curve is affected by the star-dust geometry within a galaxy, leading to more complex relationship between the observed and intrinsic galaxy emission. Using observations to stars in nearby galaxies, astronomers have derived different dust extinction curves. The most common of them are the Calzetti starburst curve, the SMC curve and the Milky Way (MW) curve which are commonly used to correct for dust attenuation in local and high-redshift galaxies. In this section we compare the attenuation of curve of the \flares\ galaxies to these most commonly used ones. In \flares\ we adopted an attenuation curve which was similar to the SMC curve, but less steep of the form:
\begin{equation}\label{eq: att_curve}
	\centering
	\tau_{\lambda} \propto \lambda^{-1}.
\end{equation}

\begin{figure*}
	\includegraphics[width=0.95\textwidth]{figures/att_curve_z5_10_Afuv.png}
	\caption{Galaxy attenuation curve for different UV attenuation. \label{fig: att_curve}}
\end{figure*}

Figure~\ref{fig: att_curve}, shows the shape of the attenuation curve for the \flares\ galaxies at $z\in[5,10]$ in different observed FUV bins. One immediate insight is that the attenuation curve gets steeper with decrease in the far-UV attenuation. The Calzett-starburst curve is more in line with highly attenuated galaxies, while the our default curve and the SMC curve agrees better with the least attenuated galaxies. 
